High Fidelity Modeling of Aerosol Pathogen Propagation in Built Environments with Moving Pedestrians

A high fidelity model for the propagation of pathogens via aerosols in the presence of moving pedestrians is proposed. The key idea is the tight coupling of computational fluid dynamics and computational crowd dynamics in order to capture the emission, transport and inhalation of pathogen loads in space and time. An example simulating pathogen propagation in a narrow corridor with moving pedestrians clearly shows the considerable effect that pedestrian motion has on airflow, and hence on pathogen propagation and potential infectivity.

==> submit.tex <==
nternational Journal for Numerical Methods in Biomedical Engineering - Manuscript # CNM-Sep-20-0220
Vijayalakshmi Viswanathan <onbehalfof@manuscriptcentral.com>
Wed 9/2/2020 8:28 PM
02-Sep-2020 Dear Prof. Lohner Your manuscript entitled "HIGH FIDELITY MODELING OF AEROSOL PATHOGEN PROPAGATION IN BUILT ENVIRONMENTS WITH MOVING PEDESTRIANS" has been successfully submitted online and is presently being given full consideration for publication in the International Journal for Numerical Methods in Biomedical Engineering. Your manuscript # is CNM-Sep-20-0220 Please mention the above manuscript # in all future correspondence regarding this submission. You can view the status of your manuscript at any time by checking your Author Centre after logging into https://secure-web.cisco.com/1VVyQvPLm37QbKjR4WDyouUsgvuJc8mDd0jbazEaoUh5_0-vJPXn3OpmtQtoTP_epqHaAdUkkI3E-rAZlKTwXyOJGq2e6nGrx9q2Xmwk_MCYdo7B454kXRHRobDltUconNkWBJfTDcEhekFbwRO0k_9668VMl2l9Y_eA0Aqk_yKzdddXtLy5s9W0hCN2aFRB66V9mvIgKahRTs2rpYtET6IWs-kVDKv1tp7YNaidwvkKO9Gm4N7CGI8sLrwY3dOfZnpnK7_Sg3hOPA3OtBjpeYkmcVSu-R8VwKKJG8CDQ-lNJZIUuwtxW4WobCL6N2ld0GSGnx9Bw6JCINHhoXhuPkjBoa5cJvQhAFDbypcVWUM8x4XWGZUEI2kwvX54EFjumcenrEItWHhXslUwwx3uD9weG7Nzk1xCLEKyJO2w7AAO0nGI9rtm60Exfg98yssj7/https%3A%2F%2Fmc.manuscriptcentral.com%2Fcnm. If you have difficulty using this site, please contact our Support Desk at support@clarivate.com. Thank you for submitting your manuscript to International Journal for Numerical Methods in Biomedical Engineering. Sincerely, International Journal for Numerical Methods in Biomedical Engineering Editorial Office ============================================================================
Find the very latest papers (ahead of the published issue of IJNMBE) via our Early View service:

http://onlinelibrary.wiley.com/journal/10.1002/(ISSN)2040-7947/earlyview

